Invariant Causal Prediction for Block MDPs

Generalization across environments is critical to the successful application of reinforcement learning algorithms to real-world challenges. In this paper, we consider the problem of learning abstractions that generalize in block MDPs, families of environments with a shared latent state space and dynamics structure over that latent space, but varying observations. We leverage tools from causal inference to propose a method of invariant prediction to learn model-irrelevance state abstractions (MISA) that generalize to novel observations in the multi-environment setting. We prove that for certain classes of environments, this approach outputs with high probability a state abstraction corresponding to the causal feature set with respect to the return. We further provide more general bounds on model error and generalization error in the multi-environment setting, in the process showing a connection between causal variable selection and the state abstraction framework for MDPs. We give empirical evidence that our methods work in both linear and nonlinear settings, attaining improved generalization over single- and multi-task baselines.

==> bounds.tex <==



\begin{theorem}[Lower bound on value estimation error]
Let $f_e$ be a mapping from $\mathcal{S} \rightarrow \mathcal{X}$. If $\exists $ $e, e', s, s'$ such that $f_e(s) = f_{e'}(s')$ (i.e. different states induce the same observation), then the following bound is a lower bound on the error obtained by a joint state abstraction over all environments, where $\delta = \min_{s, s'|f_e(s) = f_e'(s')} |v(s) - v(s')|$,

\begin{align*}
\frac{1}{|E|} \sum_{e \in E} err(\phi(X_e)) %&\geq \delta P(\phi(x) \neq f_e^{-1}(x))\\
&\ge \delta \frac{H(S|X) - 1}{\log |S|}.
\end{align*}
\end{theorem}

% \cite{luo2018algorithmic} provides more useful bounds in our setting that do not depend on the representation of the state space
% \begin{equation}
    
% \end{equation}

% \amy{\cite{gelada2019deepmdp} for bounds on value functions based on model error.}

==> figures/causal.tex <==
\begin{tikzpicture}[scale=0.75, >=stealth]
\tikzstyle{empty}=[]
\tikzstyle{obs}=[circle, inner sep=1pt, minimum size = 10mm, thick, draw =black!80, node distance = 20mm, scale=0.75]
\tikzstyle{lat}=[circle, fill =black!25, inner sep=1pt, minimum size = 10mm, thick, draw =black!80, node distance = 20mm, scale=0.75]
\tikzstyle{det}=[rectangle, fill =black, inner sep=1pt, text=white, minimum size = 6mm, draw=none, node distance = 20mm, scale=0.75]
\tikzstyle{sca}=[regular polygon,regular polygon sides=9, fill =red!50, inner sep=1pt, minimum size = 13mm, thick, draw =black!80, node distance = 20mm, scale=0.75]
\tikzstyle{connect}=[-latex, thick]
\tikzstyle{undir}=[thick]
\tikzstyle{directed}=[->, thick, shorten >=0.5 pt, shorten <=1 pt]

\node[obs] at (0.0,0.0) (x2_t)   {$X^{t}_{2}$};
\node[sca] at (1.0,2.0) (r_t)    {$R^{t}$};
\node[obs] at (0.0,4.0) (x1_t)   {$X^{t}_{1}$};

\node[obs] at (4.0,0.0) (x2_tp1) {$X^{t+1}_{2}$};
\node[sca] at (5.0,2.0) (r_tp1)  {$R^{t+1}$};
\node[obs] at (4.0,4.0) (x1_tp1) {$X^{t+1}_{1}$};

% \node      at (6.0,0.0) (x2_tp2) {$\cdots$};
% \node      at (6.0,2.0) (r_tp2) {$\cdots$};
% \node      at (6.0,4.0) (x1_tp2) {$\cdots$};

\path   
        (x1_t)   edge [directed] (r_t)
        (r_t)    edge [directed] (x2_t)
        (x1_t)   edge [directed] (x1_tp1)
        (x1_tp1) edge [directed] (r_tp1)
        (r_tp1)  edge [directed] (x2_tp1)
        % (x1_tp1) edge [directed] (x1_tp2)
        ;
\end{tikzpicture}

==> identifiability.tex <==
We now address the assumptions necessary for a model-irrelevant abstraction on a set of MDPs to also be the causal set.
This will then allow us to provide an upper bound on $W_2(\pi_{\phi(M)}, \pi_{\phi(M')})$. This requires a diversity of tasks to guarantee identifiability of the correct, minimal representation of the causal state $S$. We use the same MDP and causal graph setup as in Theorem~\ref{thm:causalstate_modelirrelevance}. 
\begin{theorem}
$S$ is identifiable if there is at least one intervention on each variable in the set $S_{K\setminus AN(R)}:=\{1,...,k\} \setminus S$. 
This means in the training set of environments there exists two environments $i, j$ where $q^i_m\neq q^j_m$ for each $m\in S_{K\setminus R}$ where $q^i_m$ is the (possibly random) function mapping the state $s$ to the variable $m$ in environment $i$. 

\end{theorem}
Proof found in \cref{app:proofs}.
Identifiability of the causal variables means that one can obtain high-probability guarantees on the generalization performance of the state abstraction while only training on a number of tasks linear in the size of the state. Our notion of intervention, namely a change in the emission function in the block MDP, contains both the hard intervention setting, where the emission function maps the particular variable to a fixed value, and the soft intervention setting, where the distribution of the variable is changed according to its emission function $q$.


